Various Types of Comet Languages and their Application in External Contextual Grammars

In this paper, we continue the research on the power of contextual grammars with selection languages from subfamilies of the family of regular languages. We investigate various comet-like types of languages and compare such language families to some other subregular families of languages (finite, monoidal, nilpotent, combinational, (symmetric) definite, ordered, non-counting, power-separating, suffix-closed, commutative, circular, or union-free languages). Further, we compare the language families defined by these types for the selection with each other and with the families of the hierarchy obtained for external contextual grammars. In this way, we extend the existing hierarchy by new language families.

==> eptcsdata.tex <==
\providecommand{\firstpage}{118}
\providecommand{\publicationstatus}{Giovanni Pighizzini, Florin Manea (Eds.): NCMA 2024\\
EPTCS 407, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.407.9}{10.4204/EPTCS.407.9}}

